Learn from What We HAVE: History-Aware VErifier that Reasons about Past Interactions Online

We introduce a novel History-Aware VErifier (HAVE) to disambiguate uncertain scenarios online by leveraging past interactions. Robots frequently encounter visually ambiguous objects whose manipulation outcomes remain uncertain until physically interacted with. While generative models alone could theoretically adapt to such ambiguity, in practice they obtain suboptimal performance in ambiguous cases, even when conditioned on action history. To address this, we propose explicitly decoupling action generation from verification: we use an unconditional diffusion-based generator to propose multiple candidate actions and employ our history-aware verifier to select the most promising action by reasoning about past interactions. Through theoretical analysis, we demonstrate that employing a verifier significantly improves expected action quality. Empirical evaluations and analysis across multiple simulated and real-world environments including articulated objects, multi-modal doors, and uneven object pick-up confirm the effectiveness of our method and improvements over baselines. Our project website is available at: https://liy1shu.github.io/HAVE_CoRL25/

==> tables/fr_train-val.tex <==
\begin{table*}[ht]
\newcommand{\clipart}[1]{\includegraphics[height=6mm]{tables/icons/#1.png}}
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}

\begin{tabular}{|r|c|c|cccccccccccccccccccc|}
\hline
\rule{0pt}{2.5em}
& \textbf{\underline{$\textbf{AVG}_{c}$}} & \textbf{\underline{$\textbf{AVG}_{s}$}} 
& \clipart{fridge} & \clipart{chair} & \clipart{laptop} & \clipart{stapler} & \clipart{trash} & \clipart{microwave} & \clipart{toilet} & \clipart{window} & \clipart{storage} & \clipart{kettle}
& \clipart{box} & \clipart{phone} & \clipart{dish} & \clipart{safe} & \clipart{oven} & \clipart{washer} & \clipart{table} & \clipart{pot} & \clipart{bucket} & \clipart{door} \\
\hline
\textbf{Baselines} & \multicolumn{22}{c|}{} \\
\hline
% (Insert all rows here as shown in your message)
FlowBot3D & 0.13 & 0.06 & 0.05 & \textbf{0.00} & \textbf{0.00} & 0.04 & 0.04 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.04 & 0.20 & 0.45 & 1.00 & 0.10 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.05 & \textbf{0.00} & 0.20 & 0.51 \\
FlowBotHD (w/o CC) & 0.22 & 0.11 & 0.21 & 0.05 & 0.03 & 0.28 & 0.14 & 0.20 & 0.08 & \textbf{0.00} & 0.06 & 0.20 & 0.20 & 0.20 & 0.38 & 0.33 & 0.49 & 0.10 & 0.06 & \textbf{0.00} & 0.80 & 0.57 \\
FlowBotHD (w/ CC) & 0.06 & 0.03 & 0.01 & 0.05 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.10 & \textbf{0.00} & \textbf{0.00} & \textbf{0.01} & 0.20 & \textbf{0.00} & \textbf{0.00} & 0.20 & 0.07 & 0.06 & 0.10 & \textbf{0.02} & \textbf{0.00} & \textbf{0.00} & 0.43 \\
Generator Only & 0.23 & 0.14 & 0.49 & 0.15 & \textbf{0.00} & 0.16 & 0.04 & \textbf{0.00} & 0.08 & 0.02 & 0.10 & 0.20 & 0.25 & 1.00 & 0.16 & 0.50 & 0.03 & \textbf{0.00} & 0.09 & \textbf{0.00} & 0.90 & 0.40 \\
Conditional Diffusion & 0.20 & 0.13 & 0.24 & 0.10 & \textbf{0.00} & 0.04 & 0.08 & 0.40 & 0.04 & 0.16 & 0.09 & 0.20 & 0.60 & \textbf{0.00} & 0.18 & 0.20 & 0.34 & 0.15 & 0.07 & \textbf{0.00} & 0.30 & 0.74 \\
\hline
\textbf{Ours} & \multicolumn{22}{c|}{} \\
\hline
HAVE (Ours) + GT obs flow & \textbf{0.02} & \textbf{0.02} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.04 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.02 & 0.20 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.03 & \textbf{0.00} & \textbf{0.00} & \textbf{0.02} & \textbf{0.00} & \textbf{0.00} & 0.17 \\
HAVE (Ours) + Estimated obs flow & 0.03 & 0.02 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.04 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.02 & 0.20 & 0.05 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.03 & \textbf{0.00} & 0.10 & \textbf{0.11} \\
\hline
\textbf{Ours (Oracle)} & \multicolumn{22}{c|}{} \\
\hline
HAVE (Ours) + Oracle Sampler & 0.02 & 0.01 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.01 & 0.20 & 0.05 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.02} & \textbf{0.00} & \textbf{0.00} & 0.06 \\
% Oracle Scoring & 0.02 & 0.02 & \textbf{0.00} & \textbf{0.00} & 0.03 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.02 & 0.16 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.07 & \textbf{0.00} & \textbf{0.00} & 0.02 & \textbf{0.00} & \textbf{0.00} & 0.11 \\
\hline
\textbf{Ablations} & \multicolumn{22}{c|}{} \\
\hline
w/o history score loss & 0.03 & 0.03 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.08 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.03 & 0.20 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.03 & \textbf{0.00} & \textbf{0.00} & 0.04 & \textbf{0.00} & 0.10 & 0.11 \\
% Uncond dataset & 0.05 & 0.03 & \textbf{0.00} & 0.25 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.20 & \textbf{0.00} & \textbf{0.00} & 0.02 & 0.20 & \textbf{0.00} & \textbf{0.00} & 0.04 & 0.10 & \textbf{0.00} & \textbf{0.00} & 0.04 & \textbf{0.00} & \textbf{0.00} & 0.20 \\
Point Cloud as Result & 0.08 & 0.04 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.08 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.01 & 0.20 & 0.50 & \textbf{0.00} & 0.10 & 0.10 & 0.06 & \textbf{0.00} & 0.04 & \textbf{0.00} & \textbf{0.00} & 0.57 \\
Sparse Action & 0.10 & 0.04 & \textbf{0.00} & 0.05 & \textbf{0.00} & 0.04 & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & 0.02 & 0.20 & 0.50 & 0.40 & 0.06 & \textbf{0.00} & 0.03 & \textbf{0.00} & 0.04 & \textbf{0.00} & 0.20 & 0.43 \\
\hline
\end{tabular}
}
\smallskip
\caption{\textbf{Failure Rate ($\downarrow$)}: Lower is better. AVG$_c$ = average over categories, AVG$_s$ = average over all samples. All 22 categories are treated as train categories. We run each object for 30 steps in simulation, and 30 samples are given for the verifier to choose from at each step. We see HAVE's overall performance increase compared with baselines and ablation choices, as well as a more balanced ability across categories.\yishu{Are the zeros kind of weird?} 
% \dave{Bold the best number in each column}
\dave{Multiply all numbers by 100 and reporting percentages}} % \dave{Maybe show a separate analysis with only failure history?}} 
\label{tab:failure-all}
\vspace*{-10pt}
\end{table*}

==> tables/sr_train-val-unseen_train.tex <==
\begin{table*}[ht]
\newcommand{\clipart}[1]{\includegraphics[height=6mm]{tables/icons/#1.png}}
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}

\begin{tabular}{|r|c|c|cccccccccc|}
\hline
\rule{0pt}{2.5em}
& \textbf{\underline{$\textbf{AVG}_{c}$}} & \textbf{\underline{$\textbf{AVG}_{s}$}} 
& \clipart{fridge} & \clipart{chair} & \clipart{laptop} & \clipart{stapler} & \clipart{trash} & \clipart{microwave} & \clipart{toilet} & \clipart{window} & \clipart{storage} & \clipart{kettle} \\
\hline
\textbf{Baselines} & \multicolumn{12}{c|}{} \\
\hline
FlowBot3D & 0.05 & 0.06 & 0.00 & 0.00 & 0.00 & 0.08 & 0.16 & 0.00 & 0.00 & 0.00 & 0.05 & 0.20 \\
FlowBotHD (w/o CC) & & & & & & & & & & & & \\
FlowBotHD (w/ CC) & & & & & & & & & & & & \\
Conditional Diffusion (CFG) & & & & & & & & & & & & \\
Generator Only & 0.10 & 0.08 & 0.24 & 0.05 & 0.05 & 0.12 & 0.26 & 0.00 & 0.02 & 0.00 & 0.10 & 0.16 \\
HAVE (Ours) + DELTA & & & & & & & & & & & & \\
HAVE (Ours) + GT obs flow & 0.04 & 0.04 & 0.00 & 0.10 & 0.00 & 0.04 & 0.02 & 0.00 & 0.00 & 0.00 & 0.01 & 0.20 \\
\hline
Oracle Sampler & 0.03 & 0.04 & 0.00 & 0.05 & 0.00 & 0.12 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.16 \\
Oracle Scoring & 0.02 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.02 & 0.16 \\
\hline
\end{tabular}
}
\smallskip
\caption{Failure Rate Results on \textbf{Train Categories} ($\downarrow$): Lower is better. AVG$_c$ is the category-wise average, AVG$_s$ is sample-wise average.}
\label{tab:success-train}
\vspace*{-10pt}
\end{table*}
